Denotationally Correct, Purely Functional, Efficient Reverse-mode Automatic Differentiation

Reverse-mode differentiation is used for optimization, but it introduces references, which break the purity of the underlying programs, making them notoriously harder to optimize. We present a reverse-mode differentiation on a purely functional language with array operations. It is the first one to deliver a provably efficient, purely functional, and denotationally correct reverse-mode differentiation. We show that our transformation is semantically correct and verifies the cheap gradient principle. Inspired by PROPs and compilation to categories, we introduce a novel intermediate representation that we call 'unary form'. Our reverse-mode transformation is factored as a compilation scheme through this intermediate representation. We obtain provably efficient gradients by performing general partial evaluation optimizations after our reverse-mode transformation, as opposed to manually derived ones. For simple first-order programs, the obtained output programs resemble static-single-assignment (SSA) code. We emphasize the modularity of our approach and show how our language can easily be enriched with more optimized primitives, as required for some speed-ups in practice.

==> figures/__latexindent_temp.tex <==
\begin{figure*}[t]
    \begin{tabular}{r c l}
        $\Dsynrevsymbol_{\rho}$(!A1,...,An!) &=& !A1,...,An,(A1x...xAn)->!$\rho$
    \end{tabular}
    
    \medskip
    \begin{tabular}{r c l}
    $\Dsynrevsymbol_{\rho}$(!var!$_{\Gamma,i}$) &=& !<var!$_{\Gamma,i}$!, J!$^T$!var!$_{\Gamma,i}$!>! \\
    $\Dsynrevsymbol_{\rho}$(!op!$_{\Gamma,n}$) &=& !<op!$_{\Gamma,n}$!, J!$^T$!op!$_{\Gamma,n}$!>! \\ 
    $\Dsynrevsymbol_{\rho}$(!e1;e2!) &=& $\Dsynrevsymbol$(!e1!); $\Dsynrevsymbol$(!e2!)\\ 
    $\Dsynrevsymbol_{\rho}$(!map2!$_{x,y.e}$) &=& !<map2!$_{x,y.e}$!, J!$^T$!map2!$_{x,y.e}$!>! \\ 
    $\Dsynrevsymbol_{\rho}$(!reduce!$_{x,y.e}$) &=& !<reduce!$_{x,y.e}$!, J!$^T$!reduce!$_{x,y.e}$!>! \\  
    \end{tabular}
    \caption{Reverse-mode differentiation from Source UNF to Target UNF}
    \label{fig:diff_macro}    
\end{figure*}

==> figures/generalisation_source_grammar.tex <==
\begin{figure*}[t]
    \setlength{\tabcolsep}{0.3em}
    \centering
    \begin{tabular}{|l c l|l|}
    \hline
    \multicolumn{3}{|c|}{\textbf{Core Grammar}} & \multicolumn{1}{c|}{\textbf{Description}}\\\hline
    !T! & \mbox{::=} & $\ldots$ & \grammarcomment{Same as before} \\
    & $\mid$ & $\Array{T}{n}$ & \grammarcomment{General Array Type}\\
    \hline
    !e! & \mbox{::=} & $\ldots$ & \grammarcomment{Same as before} \\
    & $\mid$ & !if b then e else e! & \grammarcomment{Conditionals}\\
    \hline
    \end{tabular}
    \vspace{-0.2cm}
    \caption{Grammar of the extended source language.}
    \label{fig:extended_source_grammar}
    \end{figure*}
    

==> figures/generalisation_source_typesystem.tex <==
\begin{figure*}[tb]
    \centering

    \vspace{-0.2cm}
    \caption{Type system of the extended source language}
    \vspace{-0.4cm}
    \label{fig:extended_source_typesystem}
    \end{figure*}

==> figures/generalisation_target_grammar.tex <==
\begin{figure*}[t]
    \setlength{\tabcolsep}{0.3em}
    \centering
    \begin{tabular}{|l c l|l|}
    \hline
    \multicolumn{3}{|c|}{\textbf{Core Grammar}} & \multicolumn{1}{c|}{\textbf{Description}}\\\hline
    !T! & \mbox{::=} & $\ldots$ & \grammarcomment{Real Type} \\
    \hline
    !e! & \mbox{::=} & !x! & \grammarcomment{Variable}\\
    \hline
    \end{tabular}
    \vspace{-0.2cm}
    \caption{Grammar of the extended target language.}
    \label{fig:extended_target_grammar}
    \end{figure*}

==> figures/generalisation_target_typesystem.tex <==
\begin{figure*}[tb]
    \centering

    \vspace{-0.2cm}
    \caption{Type system of the extended target language}
    \vspace{-0.4cm}
    \label{fig:extended_target_typesystem}
    \end{figure*}
